Testing Radiative Neutrino Mass Models at the LHC

The Large Hadron Collider provides us new opportunities to search for the origin of neutrino mass. Beyond the minimal see-saw models a plethora of models exist which realise neutrino mass at tree- or loop-level, and it is important to be sure that these possibilities are satisfactorily covered by searches. The purpose of this paper is to advance a systematic approach to this problem. Majorana neutrino mass models can be organised by SM-gauge-invariant operators which violate lepton number by two units. In this paper we write down the minimal ultraviolet completions for all of the mass-dimension 7 operators. We predict vector-like quarks, vector-like leptons, scalar leptoquarks, a charged scalar, and a scalar doublet, whose properties are constrained by neutrino oscillation data. A detailed collider study is presented for $O_3=LLQ\bar dH$ and $O_8 = L\bar d\bar e^\dagger \bar u^\dagger H$ completions with a vector-like quark $\chi\sim(3, 2, -\frac{5}{6})$ and a leptoquark $\phi\sim(\bar 3,1,\frac{1}{3})$. The existing LHC limits extracted from searches for vector-like fermions and sbottoms/stops are $m_\chi \gtrsim 620$ GeV and $m_\phi\gtrsim 600$ GeV.

==> FFFF.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node (d1) {};
 \node[vertex] (v1) [below right=of d1] {};
 \node[external] (d2) [below left=of v1] {};

 \node[vertex] (v2) [right=of v1] {};
 \node[vertex] (v3) [right=of v2] {};
\node[external] (b) [below=of v2] {};
 
\node[external] (nua) [above right=of v3]  {};
 \node[external] (nub) [below right=of v3]  {};
\draw[mfermion] (nua) -- (v3);
\draw[mfermion] (v3) -- (nub);
 \draw[mfermion] (d1) -- (v1);
 \draw[mfermion] (d2) -- (v1);
\draw[rscalar,red] (v1) -- (v2);
\draw[rscalar,red] (v2) -- (v3);
\draw[rscalar] (v2) -- (b);
\end{fmdg}


==> FFHH.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node (d1) {};
 \node[vertex] (v1) [below right=of d1] {};
 \node[external] (d2) [below left=of v1] {};

 \node[vertex] (v2) [right=of v1] {};
 \node[vertex] (v3) [right=of v2] {};
\node[external] (b) [below=of v2] {};


\node[external] (b2) [above=of v2] {};
 
\node[external] (nua) [above right=of v3]  {};
 \node[external] (nub) [below right=of v3]  {};
 
\draw[rscalar] (nua) -- (v3);
\draw[rscalar] (v3) -- (nub);
 \draw[mfermion] (d1) -- (v1);
 \draw[mfermion] (d2) -- (v1);
\draw[rscalar,red] (v1) -- (v2);
\draw[rscalar,red] (v2) -- (v3);
\draw[rscalar] (v2) -- (b);
\draw[rscalar] (v2) -- (b2);
\end{fmdg}


==> FFHHH.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node (d1) {};
 \node[vertex] (v1) [below right=of d1] {};
 \node[external] (d2) [below left=of v1] {};

 \node[vertex] (v2) [right=of v1] {};
 \node[vertex] (v3) [right=of v2] {};
\node[external] (b) [below=of v2] {};
 
\node[external] (nua) [above=of v3]  {};
 \node[external] (nub) [below=of v3]  {};
  \node[external] (nuc) [right=of v3]  {};
 
\draw[rscalar] (nua) -- (v3);
\draw[rscalar] (v3) -- (nub);
\draw[rscalar] (v3) -- (nuc);
 \draw[mfermion] (d1) -- (v1);
 \draw[mfermion] (d2) -- (v1);
\draw[rscalar,red] (v1) -- (v2);
\draw[rscalar,red] (v2) -- (v3);
\draw[rscalar] (v2) -- (b);
\end{fmdg}


==> FHFF.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node (d1) {};
 \node[vertex] (v1) [below right=of d1] {};
 \node[external] (d2) [below left=of v1] {};

 \node[vertex] (v2) [right=of v1] {};
 \node[vertex] (v3) [right=of v2] {};
\node[external] (b) [below=of v2] {};
 
\node[external] (nua) [above right=of v3]  {};
 \node[external] (nub) [below right=of v3]  {};
\draw[mfermion] (nua) -- (v3);
\draw[mfermion] (v3) -- (nub);
 \draw[mfermion] (d1) -- (v1);
 \draw[rscalar] (d2) -- (v1);
\draw[mfermion,red] (v1) -- (v2);
\draw[rscalar,red] (v2) -- (v3);
\draw[mfermion] (v2) -- (b);
\end{fmdg}


==> FHHHH.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node (d1) {};
 \node[vertex] (v1) [below right=of d1] {};
 \node[external] (d2) [below left=of v1] {};

 \node[vertex] (v2) [right=of v1] {};
 \node[vertex] (v3) [right=of v2] {};
\node[external] (b) [below=of v2] {};
 
\node[external] (nua) [above=of v3]  {};
 \node[external] (nub) [below=of v3]  {};
  \node[external] (nuc) [right=of v3]  {};
 
\draw[rscalar] (nua) -- (v3);
\draw[rscalar] (v3) -- (nub);
\draw[rscalar] (v3) -- (nuc);
 \draw[mfermion] (d1) -- (v1);
 \draw[rscalar] (d2) -- (v1);
\draw[mfermion,red] (v1) -- (v2);
\draw[rscalar,red] (v2) -- (v3);
\draw[mfermion] (v2) -- (b);
\end{fmdg}


==> NuMass.fmdg.tex <==
\begin{fmdg}
 \node[external] (nua) {$L_\alpha$};
 \node[vertex] (v1) [right=of nua] {};
\node[vertex] (v1a) [right=0.7cm of v1] {}; %at ($(v1)!0.5!(v2)$) {};
 \node[vertex] (v2) [right=0.7cm of v1a] {};
\node[mass] (v3a) [right=0.7cm of v2] {}; %at ($(v2)!0.5!(v3)$) {};
 \node[vertex] (v3) [right=0.7cm of v3a] {};
 \node[external] (nub) [right=of v3]  {$L_\beta$};
 \node (v4) [above=of v2] {$\phi$};
\draw[scalar] (v3.center) to[in=0,out=90] (v4.north) to[in=90,out=180] (v1.center); %to node[midway,plabel] {$\phi$} (v1.center);
  \draw[fermion] (nua) -- (v1.center);
 \draw[fermion] (v1a.center) -- node[midway,swap,plabel] {$Q_i$}(v1.center);
 \draw[fermion] (v1a.center) --node[midway,plabel] {$\bar d$} (v2.center);
  \draw[fermion] (nub) -- (v3.center);
  \draw[fermion] (v3a.center) -- node[midway,plabel] {$\bar \chi$}(v3.center);
  \draw[fermion] (v3a.center) -- node[midway,swap,plabel] {$\chi$}(v2.center);

 \node[vev,label=below left:$\braket{H}$] (vev1) [below=0.7cm of v1a] {};
  \node[vev,label=below right:$\braket{H}$] (vev3) [below=0.7cm of v2] {};

 \draw[scalar] (vev1.center) -- (v1a.center);
 \draw[scalar] (vev3.center) -- (v2.center);

\end{fmdg}


==> NuMass2.fmdg.tex <==
\begin{fmdg}

\node[vertex] (v) {};

\node[external] (L1) [left=1cm of v] {$L_\alpha$};
\draw[fermion] (L1) -- (v);

\node[vertex] (v2b) [above=0.5cm of v] {};
\node[vertex] (v2) [above=0.5cm of v2b] {};
\node[vertex] (v3) [right=1cm of v] {};
\draw[fermion] (v2b) --(v) node[midway,plabel,swap] {$\bar\chi$};
\draw[fermion] (v2b) --(v2) node[midway,plabel] {$\chi$};
\draw[scalar] (v) --(v3) node[midway,plabel] {$\phi$};

\node[external] (H) [left=of v2] {$\braket{H}$};
\draw[scalar] (H) -- (v2);

\node[vertex] (vH) [above right=1.5cm of v2] {};
\node[external]  (H2) [above=0.5cm of vH] {$\braket{H}$};
\draw[scalar] (H2) -- (vH);
\draw[fermion] (vH)  to[out=180, in=90] node [plabel,midway,swap,sloped] {$\bar d$}  (v2);

\node[vertex] (u1) [above right=0.75cm of v3] {};
\node[external] (H3) [above left=0.5cm of u1] {$\braket{H}$};
\draw[scalar] (H3) -- (u1);
\draw[fermion] (v3) -- node[midway,plabel] {$\bar u$} (u1);

\node[vertex] (u2) [right=0.75cm of u1] {};
\draw[fermion] (u2) -- node[midway,plabel,swap] {$Q$} (u1);
\draw[fermion] (vH) to[out=0,in=90] node[midway,plabel] {$Q$} (u2);

\node[vertex] (w1) [below right=0.75cm of v3] {};
\draw[fermion] (v3) -- node[midway,plabel,swap] {$\bar e$} (w1);
\node[external] (H4) [below left=0.5cm of w1] {$\braket{H}$};
\draw[scalar] (w1) --(H4);

\node[vertex] (w2) [right=0.75cm of w1] {};
\draw[fermion] (w2) -- node[midway,plabel] {$L$} (w1);
\node[external] (L2) [right=0.75cm of w2] {$L_\beta$};
\draw[fermion] (L2) -- (w2);

\draw[gaugeboson] (w2) -- node[plabel,midway,swap] {$W$} (u2);

\end{fmdg}

%  \node[external] (nua) {$L_\alpha$};
%  \node[vertex] (v1) [right=of nua] {};
% \node[vertex] (v1a) [right=0.7cm of v1] {}; %at ($(v1)!0.5!(v2)$) {};
%  \node[vertex] (v2) [right=0.7cm of v1a] {};
% \node[mass] (v3a) [right=0.7cm of v2] {}; %at ($(v2)!0.5!(v3)$) {};
%  \node[vertex] (v3) [right=0.7cm of v3a] {};
%  \node[external] (nub) [right=of v3]  {$L_\beta$};
%  \node (v4) [above=of v2] {$\phi$};
% \draw[scalar] (v3.center) to[in=0,out=90] (v4.north) to[in=90,out=180] (v1.center); %to node[midway,plabel] {$\phi$} (v1.center);
%   \draw[fermion] (nua) -- (v1.center);
%  \draw[fermion] (v1a.center) -- node[midway,swap,plabel] {$Q_i$}(v1.center);
%  \draw[fermion] (v1a.center) --node[midway,plabel] {$\bar d$} (v2.center);
%   \draw[fermion] (nub) -- (v3.center);
%   \draw[fermion] (v3a.center) -- node[midway,plabel] {$\bar \chi$}(v3.center);
%   \draw[fermion] (v3a.center) -- node[midway,swap,plabel] {$\chi$}(v2.center);

%  \node[vev,label=below left:$\braket{H}$] (vev1) [below=0.7cm of v1a] {};
%   \node[vev,label=below right:$\braket{H}$] (vev3) [below=0.7cm of v2] {};

%  \draw[scalar] (vev1.center) -- (v1a.center);
%  \draw[scalar] (vev3.center) -- (v2.center);

% \end{fmdg}


==> O2nuMass.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node[blob] (v) {};
 \node[external] (L1) [below left=of v] {$L$};
 \node[external] (L2) [below right=of v] {$L$};
 \node[external] (H) [right=of v] {$H$};

 \node[vertex] (vH) [above=of v] {};

 \node[external]  (H2) [above=0.5cm of vH] {$H$};


\draw[fermion] (L1) -- (v);
\draw[fermion] (L2) -- (v);
\draw[scalar] (H) -- (v);
\draw[scalar] (H2) -- (vH);

\draw[fermion,bend left] (vH)  to[out=-90, in=-135] node [plabel,midway,sloped,swap] {$L$}  (v);
\draw[fermion,bend right] (vH) to[out=90,in=135]  node [plabel,midway,sloped] {$\bar e$} (v);

\end{fmdg}


==> O3anuMass.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node[blob] (v) {};
 \node[external] (L1) [below left=1.5cm of v] {$L$};
 \node[vertex] (L2p) [below right=0.75cm of v] {};
 \node[external] (L2) [below right=1.5cm of v] {$L$};
 \node[vertex] (Hp) [right=0.75cm of v] {};
 \node[external] (H) [right=1.5cm of v] {$H$};

 \node[vertex] (vH) [above=of v] {};

 \node[external]  (H2) [above=0.5cm of vH] {$H$};


\draw[fermion] (L1) -- (v);
\draw[fermion] (L2p) -- node[plabel,pos=0.3,sloped] {$L$} (v) ;
\draw[fermion] (L2) -- (L2p);
\draw[scalar] (Hp) -- node[plabel,midway,sloped,swap] {$H$} (v);
\draw[scalar] (H) -- (Hp);
\draw[scalar] (H2) -- (vH);

\draw[gaugeboson] (L2p) -- node[plabel,midway,swap] {$W$} (Hp);

\draw[fermion,bend left] (vH)  to[out=-90, in=-135] node [plabel,midway,sloped,swap] {$Q$}  (v);
\draw[fermion,bend right] (vH) to[out=90,in=135]  node [plabel,midway,sloped] {$\bar d$} (v);

\end{fmdg}


==> O3anuMass2.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node[blob] (v) {};
 \node[vertex] (L2p) [below left=0.75cm of v] {};
 \node[external] (L1) [below left=1.5cm of v] {$L$};
 \node[external] (L2) [below right=1.5cm of v] {$L$};

 \node[vertex] (Hp) [right=0.75cm of v] {};
 \node[external] (H) [right=1.5cm of v] {$H$};

 \node[vertex] (vH) [above=of v] {};

 \node[external]  (H2) [above=0.5cm of vH] {$H$};


\draw[fermion] (L2) -- (v);
\draw[fermion] (L2p) -- node[plabel,pos=0.3,sloped,swap] {$L$} (v) ;
\draw[fermion] (L1) -- (L2p);
%\draw[scalar] (Hp) -- node[plabel,midway,sloped,swap] {$H$} (v);
\draw[scalar] (H) -- (v);
\draw[scalar] (H2) -- (vH);

\node[vertex] (Hp) at (-0.7,1) {}; 

\draw[gaugeboson] (L2p) to[out=90,in=215] node[plabel,midway] {$W$} (Hp);


\draw[fermion,bend left] (vH)  to[out=-30, in=225]  node [plabel,midway,sloped,swap] {$Q$} (Hp);

\draw[fermion,bend left] (Hp)  to[out=-45, in=-135]  node [plabel,midway] {$Q$} (v);


\draw[fermion,bend right] (vH) to[out=90,in=135]  node [plabel,midway,sloped] {$\bar d$} (v);


\end{fmdg}


==> O3bnuMass.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
 \node[blob] (v) {};
 \node[external] (L1) [below left=of v] {$L$};
 \node[external] (L2) [below right=of v] {$L$};
 \node[external] (H) [right=of v] {$H$};

 \node[vertex] (vH) [above=of v] {};

 \node[external]  (H2) [above=0.5cm of vH] {$H$};


\draw[fermion] (L1) -- (v);
\draw[fermion] (L2) -- (v);
\draw[scalar] (H) -- (v);
\draw[scalar] (H2) -- (vH);

\draw[fermion,bend left] (vH)  to[out=-90, in=-135] node [plabel,midway,sloped,swap] {$Q$}  (v);
\draw[fermion,bend right] (vH) to[out=90,in=135]  node [plabel,midway,sloped] {$\bar d$} (v);

\end{fmdg}


==> O8nuMass.fmdg.tex <==
%!TeX root=draft.tex
\begin{fmdg}
\node[blob] (v) {};

\node[external] (L1) [below left=1.5cm of v] {$L$};
\draw[fermion] (L1) -- (v);

\node[external] (H) [left=of v] {$H$};
\draw[scalar] (H) -- (v);

\node[vertex] (vH) [above=1.5cm of v] {};
\node[external]  (H2) [above=0.5cm of vH] {$H$};
\draw[scalar] (H2) -- (vH);
\draw[fermion] (vH)  to[out=180, in=135] node [plabel,midway,swap,sloped] {$\bar d$}  (v);

\node[vertex] (u1) [above right=0.75cm of v] {};
\node[external] (H3) [above left=0.5cm of u1] {$H$};
\draw[scalar] (H3) -- (u1);
\draw[fermion] (v) -- node[midway,plabel,swap] {$\bar u$} (u1);

\node[vertex] (u2) [right=0.75cm of u1] {};
\draw[fermion] (u2) -- node[midway,plabel] {$Q$} (u1);
\draw[fermion] (vH) to[out=0,in=90] node[midway,plabel] {$Q$} (u2);

\node[vertex] (w1) [below right=0.75cm of v] {};
\draw[fermion] (v) -- node[midway,plabel] {$\bar e$} (w1);
\node[external] (H4) [below=0.5cm of w1] {$H$};
\draw[scalar] (w1) --(H4);

\node[vertex] (w2) [right=0.75cm of w1] {};
\draw[fermion] (w2) -- node[midway,plabel] {$L$} (w1);
\node[external] (L2) [below right=0.75cm of w2] {$L$};
\draw[fermion] (L2) -- (w2);

\draw[gaugeboson] (w2) -- node[plabel,midway] {$W$} (u2);

\end{fmdg}

